On the equivalence of semi-classical methods for QED in intense external fields

Using the semi-classical method of Nikishov-Ritus (NR), the derivation of the transition rate of the beamstrahlung process is reviewed. This method uses the Bound Interaction Picture and the exact solutions of the Dirac equation in the external field potential. For future linear colliders, the nominal machine parameters are such that this external field can be considered to be a constant crossed electromagnetic field. The Dirac equation solutions can be Fourier transformed such that they are functions of Dirac gamma matrices, Airy functions and the usual non-external field solution. The resultant analytic form for the transition rate is the same as that obtained by the Quasiclassical Operator (QO) method of Baier-Katkov which sets a limit of ultra-relativistic electron and vanishingly small radiation angle. The NR calculation however also exhibits a pole in the radiation angle for back-radiated photons. The removal of this pole requires a further study of IR divergences within the Bound Interaction Picture.

==> mydefs.tex <==
%--------------------------------------------------------------------------
%    shortened versions of long commands that I can't be bothered
%    typing in all the time
%--------------------------------------------------------------------------
\newcommand{\nwcd}{\newcommand}
%-------redefinitions so emtex doesn't choke------------
\nwcd{\dint}{{\displaystyle \int}}
\nwcd{\dsum}{\sum}
\nwcd{\text}{\mbox}
\nwcd{\limfunc}{\mbox}
\nwcd{\NEG}{\slash}
\nwcd{\nts}{\negthinspace}
\nwcd{\nms}{\negmedspace}
\nwcd{\nths}{\negthickspace\negthickspace}
%\nwcd{\underrightarrow}{\vec}
%-----------------------------------------------------------
\nwcd{\vep}{\varepsilon}
\nwcd{\undl}{\underline}
\nwcd{\dd}{\ddagger}
\nwcd{\pr}{\prime}
\nwcd{\witl}{\widetilde}
\nwcd{\bm}{\pmb}
\nwcd{\mvb}{\mathversion{bold}}
%------
%---------------------------------------------------------------------------
%    define some oft used commands
%---------------------------------------------------------------------------
\nwcd{\lami}{(\lambda_{i})}
\nwcd{\lamf}{(\lambda_{f})}
%--------------------------------------------------------------------------
\renewcommand{\bar}[1]{\setbox0=\hbox{$#1$}
                       \setlength{\unitlength}{\wd0}
                       \smash{\buildrel \line(1,0){0.7} \over #1}}
%--------------------------------------------------------------------------
\def\dbr#1{\setbox0=\hbox{$#1$} 
           \setlength{\unitlength}{\wd0}
           \smash{\buildrel \overline{\line(1,0){0.7}} \over #1}}
%----------------------------------------------------------------------
\nwcd{\balph}[1]{\setbox0=\hbox{$#1$}
                       \setlength{\unitlength}{\wd0}
                       \smash{\mathrel{\mathop{\line(1,0){0.7}} \atop #1}}}
%--------------------------------------------------------------------------
\def\dalph#1{\setbox0=\hbox{$#1$} 
           \setlength{\unitlength}{\wd0}
           \smash{\mathrel{\mathop{\overline{\line(1,0){0.7}}} \atop #1}}}
%----------------------------------------------------------------------
\nwcd{\half}{{\textstyle \frac{1}{2}}}
\nwcd{\sql}[1]{#1\hspace{-1.6ex}\raisebox{-1.5ex}{$\sim$}}
\nwcd{\squ}[1]{#1\hspace{-1.5ex}\raisebox{-1.0ex}{$\sim$}}
\nwcd{\eapbf}{\frac{e^{2}a^{2}}{4(k\bar{p})(kp_{f})}}
\nwcd{\eapbi}{\frac{e^{2}a^{2}}{4(k\bar{p})(kp_{i})}}
\nwcd{\eapdbf}{\frac{e^{2}a^{2}}{4(k\dbr{p})(kp_{f})}}
\nwcd{\eapdbi}{\frac{e^{2}a^{2}}{4(k\dbr{p})(kp_{i})}}
%----------------------------------------------------------------------------
%  Now a whole lot of scalar products
%-----------------------------------------------------------------------------
\nwcd{\pipbrp}{[(p_{i}\bar{p}_{r\pr})+m^{2}]}
\nwcd{\pipbr}{[(p_{i}\bar{p}_{r})+m^{2}]}
\nwcd{\bpr}{\bar{p}_{r}}
\nwcd{\dpr}{\dbr{p}_{r\pr}}
%
%------------------------------------------------------------------------------
\nwcd{\pmsqb}{\bar{p}^{2}_{r}-m^{2}}
\nwcd{\pmsqbp}{\bar{p}^{2}_{r\prime}-m^{2}}
\nwcd{\pmsqdb}{\dbr{p}^{2}_{r}-m^{2}}
\nwcd{\pmsqdbp}{\dbr{p}^{2}_{r\prime}-m^{2}}
%\nwcd{\mat}[1]{$\; #1 \;$}
\nwcd{\gmu}{\gamma_{\mu}}
\nwcd{\gnu}{\gamma_{\nu}}
%
% ---------- Bras and kets
\def\bra#1{\langle#1\vert}              % \bra{stuff} gives <stuff|
\def\ket#1{\vert#1\rangle}              % \ket{stuff} gives |stuff>
%
% ---------- Functions -- all defined like \sin, etc. in Plain TeX:
\def\real{\mathop{\rm Re}\nolimits}     % Re for real part
\def\imag{\mathop{\rm Im}\nolimits}     % Im for imaginary part

\def\tr{\mathop{\rm tr}\nolimits}       % tr for trace
\def\Tr{\mathop{\rm Tr}\nolimits}       % Tr for functional trace
%
%--------------------------------------------------------------------------
%  \slashchar puts a slash through a character to represent contraction
%  with Dirac matrices. Use \not instead for negation of relations, and use
%  \hbar for hbar.

%\def\slash#1{\setbox0=\hbox{$#1$}               % set a box for #1
%   \dimen0=\wd0                                 % and get its size
%   \setbox1=\hbox{/} \dimen1=\wd1               % get size of /
%   \ifdim\dimen0>\dimen1                        % #1 is bigger
%      \rlap{\hbox to \dimen0{\hfil/\hfil}}      % so center / in box
%      #1                                        % and print #1
%   \else                                        % / is bigger
%      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}   % so center #1
%      /                                         % and print /
%   \fi}                                         %
%-----------------------------------------------------------------------------
%\def\slash#1{\setbox0=\hbox{$\,#1\,$}
%             \setlength{\unitlength}{\wd0}
%             \rlap{\raisebox{-0.2ex}{\line(3,2){1.0}}} \,#1}
%-----------------------------------------------------------------------------
%   defined commands using \slash
%-----------------------------------------------------------------------------
\nwcd{\gmaok}{\gamma_{\mu}\slashed{a}_{1}\slashed{k}}
\nwcd{\gmatk}{\gamma_{\mu}\slashed{a}_{2}\slashed{k}}
\nwcd{\gnaok}{\gamma_{\nu}\slashed{a}_{1}\slashed{k}}
\nwcd{\gnatk}{\gamma_{\nu}\slashed{a}_{2}\slashed{k}}
%
\nwcd{\aokgm}{\slashed{a}_{1}\slashed{k}\gamma_{\mu}}
\nwcd{\atkgm}{\slashed{a}_{2}\slashed{k}\gamma_{\mu}}
\nwcd{\aokgn}{\slashed{a}_{1}\slashed{k}\gamma_{\nu}}
\nwcd{\atkgn}{\slashed{a}_{2}\slashed{k}\gamma_{\nu}}
%
\nwcd{\pmsq}{\displaystyle \left[\frac{\slashed{p} + m}{p^{2} - m^{2}}
\right]}
\nwcd{\pbr}{\left[\frac{\slashed{\bar{p}}_{r} + m}{\bar{p}_{r}^{2} - m^{2}}
\right]}
\nwcd{\pbrp}{\left[\frac{\slashed{\bar{p}}_{r\prime} + m}{\bar{p}_{r\prime}
^{2} - m^{2}}\right]}
\nwcd{\pdbr}{\left[\frac{\slashed{\dbr{p}}_{r} + m}{\dbr{p}_{r}^{2} - m^{2}}
\right]}
\nwcd{\pdbrp}{\left[\frac{\slashed{\dbr{p}}_{r\prime} + m}{\dbr{p}_{r\prime}
^{2} - m^{2}}\right]}

